An improvement to an algorithm of Belabas, Diaz y Diaz and Friedman

In [BDyDF08] Belabas, Diaz y Diaz and Friedman show a way to determine, assuming the Generalized Riemann Hypothesis, a set of prime ideals that generate the class group of a number field. Their method is efficient because it produces a set of ideals that is smaller than earlier proved results. Here we show how to use their main result to algorithmically produce a bound that is lower than the one they prove.

==> abbrev.tex <==
\makeatletter
\def\oper#1{\expandafter\def\csname #1\endcsname{\mathop{\operator@font #1}\nolimits}}
\def\Set#1{\expandafter\def\csname #1\endcsname{{\operator@font #1}}}
\def\c@r#1#2#3{\expandafter\def\csname#1#2\endcsname{{\ensuremath{#3{#1}}}\xspace}}
\def\+#1#2{\ifx#2C\c@r#1#2{\mathcal}\else\ifx#2M\c@r#1#2{\bf}\else\ifx#2G\c@r#1#2{\mathfrak}\else\ifx#2N\c@r#1#2{\textup}\else\ifx#2S\c@r#1#2{\sf}\else\ifx#2B\c@r#1#2{\mathbb}\fi\fi\fi\fi\fi\fi%
}

\oper{arctanh}
\def\bv{\underline b}
\+CC
\+CM
\def\Cl{{\ensuremath{\CC\!\ell}}\xspace}
\def\d{\,\mathrm d}
\def\DK{{\ensuremath{\Delta_\K}}\xspace}
\def\good{$K$-good\xspace}
\oper{dilog}
\def\GRH{\textrm{\upshape GRH}\xspace}
\+IC
\let\l@icIm=\Im
\oper{Im}
\let\Imm=\Im\let\Im=\l@icIm
\def\intpart#1{\left\lfloor#1\right\rfloor}
\def\e{\varepsilon}
\oper{Ei}
\def\fracpart#1{\left\{#1\right\}}
\def\g{\gamma}
\+KM
\def\K{\KM}
\def\L{{\ensuremath{\mathrm L}}\xspace}
\def\lDK{{\ensuremath{\log\DK}}\xspace}
\def\ldp{\ensuremath{\frac{\zeta'}{\zeta}}\xspace}
\def\ldpK{\ensuremath{\frac{\zKp}{\zK}}\xspace}
\def\llDK{{\ensuremath{\log\lDK}}\xspace}
\def\N{{\ensuremath{\mathrm N}}\xspace}
\def\nK{{\ensuremath{n_\K}}\xspace}
\+NM
\+OC
\def\OK{{\ensuremath{\OC_K}}\xspace}
\+pG
\let\l@icRe=\Re
\oper{Re}
\let\Ree=\Re\let\Re=\l@icRe
\+QM
\+RM
\+SC
\def\tbv{{}^t\bv}
\+WC
\def\zK{{\ensuremath{\zeta_\K}}\xspace}
\def\zKp{{\ensuremath{\zeta'_\K}}\xspace}
\+ZM


==> macros.tex <==
\def\thefootnote{(\arabic{footnote})}
\makeatletter
\def\loic@eng{english}
\def\loic@ita{italian}
\ifx\languagename\loic@eng
    \def\theoname{Theorem}
    \def\propname{Proposition}
    \def\lemmname{Lemma}
    \def\definame{Definition}
    \def\coroname{Corollary}
    \def\conjname{Conjecture}
    \def\remaname{Remark}
\else\ifx\languagename\loic@ita
    \def\theoname{Teorema}
    \def\propname{Proposizione}
    \def\lemmname{Lemma}
    \def\definame{Definizione}
    \def\coroname{Corollario}
    \def\conjname{Conjecture}
    \def\remaname{Osservazione}
\else
    \def\theoname{Th\'eor\`eme}
    \def\propname{Proposition}
    \def\lemmname{Lemme}
    \def\definame{D\'efinition}
    \def\coroname{Corollaire}
    \def\conjname{Conjecture}
    \def\remaname{Remarque}
\fi\fi
%\def\newtheorem#1{%
%  \@ifnextchar[{\@othm{#1}}{\@nthm{#1}}}
%\makeatother
\newtheorem{theo}[equation]{\theoname}
%\renewcommand{\thetheo}{\arabic{theo}}
\tracingmacros2
\newtheorem{theonamed}{\theoname}
\tracingmacros0
\renewcommand{\thetheonamed}{\arabic{section}.\arabic{theonamed}}
\newtheorem{coronamed}[theonamed]{\coroname}
\newtheorem{prop}[equation]{\propname}
%\renewcommand{\theprop}{\thesection.\arabic{prop}}
\newtheorem{defi}[equation]{\definame}
%\renewcommand{\thedefi}{\thesection.\arabic{defi}}
\newtheorem{propdefi}[equation]{\propname--\definame}
%\renewcommand{\thepropdefi}{\thesection.\arabic{propdefi}}
\newcount\endpf\endpf=0\newcount\pfnum\pfnum=0
\newenvironment{preuve}[1][]%
        {\par\noindent{\sc\proofname\xspace #1}:~\ignorespaces\advance\pfnum1\global\advance\endpf1}%
        {\ifnum\pfnum=\endpf\unskip\nobreak\hskip2em plus1fill$\square$\par\medskip\global\advance\endpf-1\advance\pfnum-1\fi}
\newtheorem{coro}[equation]{\coroname}
%\renewcommand{\thecor}{\thesection.\arabic{cor}}
\newtheorem{lem}[equation]{\lemmname}
%\renewcommand{\thelem}{\thesection.\arabic{lem}}
\newtheorem{conj}[equation]{\conjname}
%\renewcommand{\theconj}{\thesection.\arabic{conj}}
%\theorembodyfont{\upshape}
\theoremstyle{remark}
\newtheorem{rem}[equation]{\remaname}
%\renewcommand{\therem}{\thesection.\arabic{rem}}
\newtheorem*{rem*}{\remaname}
\def\lpara#1{\paragraph{\bf #1}}

\let\pointdexclamation=!
\let\inferieur=<
\let\superieur=>
\let\egal==
{
\makeatletter
\catcode`!\active
\catcode`<\active
\catcode`>\active
\global\everymath={\catcode`!=\active\def!{\mathpointdexclamation}\catcode`<\active\catcode`>\active%
\def\mathpointdexclamation{\@ifnextchar\egal{\not}{\pointdexclamation}}%
\def<{\@ifnextchar\egal{\leqslant\@gobble}{\inferieur}}%
\def>{\@ifnextchar\egal{\geqslant\@gobble}{\superieur}}}
\global\everydisplay={\catcode`!\active\catcode`<\active\catcode`>\active%
\def!{\@ifnextchar\egal{\not}{\pointdexclamation}}%
\def<{\@ifnextchar\egal{\leqslant\@gobble}{\inferieur}}%
\def>{\@ifnextchar\egal{\geqslant\@gobble}{\superieur}}}
\makeatother
}

\def\aquot#1#2{\mathchoice%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\displaystyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\displaystyle #2$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\textstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\textstyle #2$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptstyle #2$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptscriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptscriptstyle #2$}}}
\def\quot#1#2{\mathchoice%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\displaystyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\displaystyle #2$}}%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\textstyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\textstyle #2$}}%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\scriptstyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\scriptstyle #2$}}%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\scriptscriptstyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\scriptscriptstyle #2$}}}
\def\biquot#1#2#3{\mathchoice%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\displaystyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\displaystyle #2$}\kern-.1em/\lower.25ex\hbox{$\displaystyle #3$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\textstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\textstyle #2$}\kern-.1em/\kern-.1em\lower.25ex\hbox{$\textstyle #3$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptstyle #2$}\kern-.1em/\kern-.1em\lower.25ex\hbox{$\scriptstyle #3$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptscriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptscriptstyle #2$}\kern-.1em/\kern-.1em\lower.25ex\hbox{$\scriptscriptstyle #3$}}}
\def\aquot#1#2{\mathchoice%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\displaystyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\displaystyle #2$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\textstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\textstyle #2$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptstyle #2$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptscriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptscriptstyle #2$}}}
\def\quot#1#2{\mathchoice%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\displaystyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\displaystyle #2$}}%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\textstyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\textstyle #2$}}%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\scriptstyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\scriptstyle #2$}}%
{\leavevmode\kern-.1em\raise.2ex\hbox{$\scriptscriptstyle #1$}\kern-.1em/\kern-.1em%
\lower.25ex\hbox{$\scriptscriptstyle #2$}}}
\def\biquot#1#2#3{\mathchoice%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\displaystyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\displaystyle #2$}\kern-.1em/\lower.25ex\hbox{$\displaystyle #3$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\textstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\textstyle #2$}\kern-.1em/\kern-.1em\lower.25ex\hbox{$\textstyle #3$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptstyle #2$}\kern-.1em/\kern-.1em\lower.25ex\hbox{$\scriptstyle #3$}}%
{\leavevmode\kern-.1em\lower.25ex\hbox{$\scriptscriptstyle #1$}\kern-.1em\backslash\kern-.1em%
\raise.2ex\hbox{$\scriptscriptstyle #2$}\kern-.1em/\kern-.1em\lower.25ex\hbox{$\scriptscriptstyle #3$}}}
\makeatother

